PiCIE: Unsupervised Semantic Segmentation using Invariance and Equivariance in Clustering

We present a new framework for semantic segmentation without annotations via clustering. Off-the-shelf clustering methods are limited to curated, single-label, and object-centric images yet real-world data are dominantly uncurated, multi-label, and scene-centric. We extend clustering from images to pixels and assign separate cluster membership to different instances within each image. However, solely relying on pixel-wise feature similarity fails to learn high-level semantic concepts and overfits to low-level visual cues. We propose a method to incorporate geometric consistency as an inductive bias to learn invariance and equivariance for photometric and geometric variations. With our novel learning objective, our framework can learn high-level semantic concepts. Our method, PiCIE (Pixel-level feature Clustering using Invariance and Equivariance), is the first method capable of segmenting both things and stuff categories without any hyperparameter tuning or task-specific pre-processing. Our method largely outperforms existing baselines on COCO and Cityscapes with +17.5 Acc. and +4.5 mIoU. We show that PiCIE gives a better initialization for standard supervised training. The code is available at https://github.com/janghyuncho/PiCIE.

==> picie_pseudocode.tex <==

\begin{algorithm}
\caption{PiCIE pseudocode}
\begin{algorithmic}
\STATE\text{RTsampler : samples random transformations.}
\STATE\text{RTlist : a list to store random transformations.}
\STATE $\mu_1, \mu_2\text{ : cluster centroids for view 1 and 2.}$
\STATE $o_1, o_2\text{ : pixel-level features for view 1 and 2.}$
\STATE $P_1, P_2, G \text{ : photometric and geometric transformations.}$
\STATE $\text{backward} \text{ : backward function with ADAM optimizer.}$
\midrule
\STATE \text{1. Produce 2 views and cluster with batch k-means.}
\FOR {$(\text{index}, x) \sim \mathcal{D}$}
\STATE $P_1, P_2, G \sim \text{RTsampler}$
\STATE $o_1 \leftarrow G(f_\theta( P_1(x)))$
\STATE $o_2 \leftarrow f_\theta(G(P_2(x)))$
\STATE $\mu_1 \leftarrow \text{BatchKMeans}(o_1, \mu_1)$
\STATE $\mu_2 \leftarrow \text{BatchKMeans}(o_2, \mu_2)$
\STATE $\text{RTlist.update}(P_1, P_2, G, \text{index})$
\ENDFOR
\STATE \text{2. Compute segmentation pseudo-labels.}
\FOR {$(\text{index}, x) \sim \mathcal{D}$}
\STATE $P_1, P_2, G \leftarrow \text{RTlist}(\text{index})$
\STATE $o_1 \leftarrow G(f_\theta( P_1(x)))$
\STATE $o_2 \leftarrow f_\theta(G(P_2(x)))$
\STATE $y_1 \leftarrow \arg\max\text{PrototypeClassifier}(o_1, \mu_1)$
\STATE $y_2 \leftarrow \arg\max\text{PrototypeClassifier}(o_2, \mu_2)$
\STATE $\mathcal{Y}\text{.update}(y_1, y_2)$
\ENDFOR 
\STATE \text{3. Cross-view training.}
\FOR {$(\text{index}, x, y_1, y_2) \sim \mathcal{D}\cup \mathcal{Y}$}
\STATE $P_1, P_2, G \leftarrow \text{RTlist}(\text{index})$
\STATE $o_1 \leftarrow G(f_\theta( P_1(x)))$
\STATE $o_2 \leftarrow f_\theta(G(P_2(x)))$
\STATE $p_{11} \leftarrow \text{PrototypeClassifier}(o_1, \mu_1)$
\STATE $p_{22} \leftarrow \text{PrototypeClassifier}(o_2, \mu_2)$
\STATE $p_{12} \leftarrow \text{PrototypeClassifier}(o_1, \mu_2)$
\STATE $p_{21} \leftarrow \text{PrototypeClassifier}(o_2, \mu_1)$
\STATE $\mathcal{L}_{\text{within}} \leftarrow \mathcal{L}_{\text{CE}}(p_{11}, y_1) + \mathcal{L}_{\text{CE}}(p_{22}, y_2)$
\STATE $\mathcal{L}_{\text{cross}} \leftarrow \mathcal{L}_{\text{CE}}(p_{12}, y_2) + \mathcal{L}_{\text{CE}}(p_{21}, y_1)$
\STATE $\mathcal{L}_{\text{total}} \leftarrow (\mathcal{L}_{\text{within}} + \mathcal{L}_{\text{cross}})/4$
\STATE $f_\theta \leftarrow \text{backward}(\mathcal{L}_{\text{total}})$
\ENDFOR 
\end{algorithmic}
\end{algorithm}


==> picie_pseudocode_simpler.tex <==
\begin{algorithm}
\caption{PiCIE pseudocode}
\begin{algorithmic}
\STATE $\mu_1, \mu_2\text{ : cluster centroids for view 1 and 2.}$
\STATE $o_1, o_2\text{ : pixel-level features for view 1 and 2.}$
\STATE $P_1, P_2, G \text{ : photometric and geometric transformations.}$
\STATE $\text{backward} \text{ : backward function with ADAM optimizer.}$
\midrule
\STATE \text{1. Produce 2 views and cluster with batch k-means.}
\FOR {$(\text{index}, x) \sim \mathcal{D}$}
\STATE $P_1, P_2, G \sim \text{RTsampler}$
\STATE $o_1 \leftarrow G(f_\theta( P_1(x)))$
\STATE $o_2 \leftarrow f_\theta(G(P_2(x)))$
\STATE $\mu_1 \leftarrow \text{BatchKMeans}(o_1, \mu_1)$
\STATE $\mu_2 \leftarrow \text{BatchKMeans}(o_2, \mu_2)$
\STATE $\text{RTlist.update}(P_1, P_2, G, \text{index})$
\ENDFOR
\STATE \text{2. Compute segmentation pseudo-labels.}
\FOR {$(\text{index}, x) \sim \mathcal{D}$}
\STATE $P_1, P_2, G \leftarrow \text{RTlist}(\text{index})$
\STATE $o_1 \leftarrow G(f_\theta( P_1(x)))$
\STATE $o_2 \leftarrow f_\theta(G(P_2(x)))$
\STATE $y_1 \leftarrow \arg\max\text{PrototypeClassifier}(o_1, \mu_1)$
\STATE $y_2 \leftarrow \arg\max\text{PrototypeClassifier}(o_2, \mu_2)$
\STATE $\mathcal{Y}\text{.update}(y_1, y_2)$
\ENDFOR 
\STATE \text{3. Cross-view training.}
\FOR {$(\text{index}, x, y_1, y_2) \sim \mathcal{D}\cup \mathcal{Y}$}
\STATE $P_1, P_2, G \leftarrow \text{RTlist}(\text{index})$
\STATE $o_1 \leftarrow G(f_\theta( P_1(x)))$
\STATE $o_2 \leftarrow f_\theta(G(P_2(x)))$
\STATE $p_{11} \leftarrow \text{PrototypeClassifier}(o_1, \mu_1)$
\STATE $p_{22} \leftarrow \text{PrototypeClassifier}(o_2, \mu_2)$
\STATE $p_{12} \leftarrow \text{PrototypeClassifier}(o_1, \mu_2)$
\STATE $p_{21} \leftarrow \text{PrototypeClassifier}(o_2, \mu_1)$
\STATE $\mathcal{L}_{\text{within}} \leftarrow \mathcal{L}_{\text{CE}}(p_{11}, y_1) + \mathcal{L}_{\text{CE}}(p_{22}, y_2)$
\STATE $\mathcal{L}_{\text{cross}} \leftarrow \mathcal{L}_{\text{CE}}(p_{12}, y_2) + \mathcal{L}_{\text{CE}}(p_{21}, y_1)$
\STATE $\mathcal{L}_{\text{total}} \leftarrow (\mathcal{L}_{\text{within}} + \mathcal{L}_{\text{cross}})/4$
\STATE $f_\theta \leftarrow \text{backward}(\mathcal{L}_{\text{total}})$
\ENDFOR 
\end{algorithmic}
\end{algorithm}

